A robust solver for elliptic PDEs in 3D complex geometries

We develop a boundary integral equation solver for elliptic partial differential equations on complex \threed geometries. Our method is efficient, high-order accurate and robustly handles complex geometries. A key component is our singular and near-singular layer potential evaluation scheme, \qbkix: a simple extrapolation of the solution along a line to the boundary. We present a series of geometry-processing algorithms required for \qbkix to run efficiently with accuracy guarantees on arbitrary geometries and an adaptive upsampling scheme based on a iteration-free heuristic for quadrature error. We validate the accuracy and performance with a series of numerical tests and compare our approach to a competing local evaluation method.

==> macros.tex <==
%% macro to define and reference terms with document
\usepackage{relsize}
\newcommand\abbrev[1]{\textsmaller{\uppercase{#1}}} %could do \textsc{\large\lowercase{#1}} or {\small\uppercase{#1}}, insert \textup to keep the letters in Roman/upright form, e.g. \abbrevformat{O\textup{\small pen}MP}

\newcommand\gmres{\abbrev{GMRES}\xspace}
\newcommand\pde{\abbrev{PDE}\xspace}
\newcommand\bvp{\abbrev{BVP}\xspace}
\newcommand\pdes{\abbrev{PDE}s\xspace}
\newcommand\ki{kernel-independent\xspace}
\newcommand\kifmm{\abbrev{KIFMM}\xspace}
\newcommand\fmm{\abbrev{FMM}\,}
\newcommand\fft{\abbrev{FFT}\,}
\newcommand\oned{\abbrev{1D}\,}
\newcommand\twod{\abbrev{2D}\,}
\newcommand\threed{\abbrev{3D}\,}
\newcommand\qbx{\abbrev{QBX}\,}
\newcommand\bie{\abbrev{BIE}\,}
\newcommand\aabb{\abbrev{AABB}\,}
\newcommand\pvfmm{\abbrev{PVFMM}\,}
\newcommand\qbkix{\texttt{hedgehog}\,}
\newcommand\pou{\abbrev{POU}\,}
\newcommand\bem{\abbrev{BEM}\,}
\newcommand\mfs{\abbrev{MFS}\,}
\newcommand\iga{\abbrev{IGA}\,}
\newcommand\wfine{\vector{w}_\text{fine}}
\newcommand\phifine{\vector{\phi}_\text{fine}}
\newcommand\Gammah{\hat{\Gamma}}
\newcommand\nystrom{Nystr\"om\xspace}


%% shortcuts (this paper) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\GL{Gauss-Legendre}
\def\Pex{\ensuremath{P_\mathrm{ex}}}
\def\Cex{\ensuremath{C_\mathrm{ex}}}
\def\Pnear{\ensuremath{P_\mathrm{near}}}
\def\Cnear{\ensuremath{C_\mathrm{near}}}
\def\Tree{\ensuremath{\mathscr T}}
\def\CenterSet{\ensuremath{\mathscr C}}
\def\PatchSet{\ensuremath{\mathscr P}}
\def\UnPatch{\ensuremath{{\mathscr U}_p}}
\def\UnBox{\ensuremath{{\mathscr U}_b}}
\def\CCover{\ensuremath{C_\mathrm{cover}}}
\def\BCover{\ensuremath{B_\mathrm{cover}}}
\def\Npatch{\ensuremath{N_\mathrm{patch}}}
\def\Ncenter{\ensuremath{N_\mathrm{center}}}
\def\Nbox{\ensuremath{N_\mathrm{box}}}
\DeclareMathOperator{\dist}{dist}


\newcommand\qP{{\mathcal{P}}}
\newcommand\I{{\mathcal{I}}}
\newcommand\Pfine{{\mathcal{P}_\lbl{fine}}}
\newcommand\Pcoarse{{\mathcal{P}_\lbl{coarse}}}
\newcommand\err[1]{{\eps_\lbl{#1}}}
\newcommand{\etrg}{\err{target}}
\newcommand\mrm[1]{\mathrm{#1}}
\let\vec\undefined
\let\vector\undefined
\newcommand\vector[1]  {\bm{#1}}
\newcommand\vx{{\vector{x}}}
\newcommand\hr{{\hat{r}}}
\newcommand\vg{{\vector{g}}}
\newcommand\vX{{\vector{X}}}
\newcommand\vP{{\vector{P}}}
\newcommand\vy{{\vector{y}}}
\newcommand\vd{{\vector{d}}}
\newcommand\vc{{\vector{c}}}
\newcommand\vhc{{\hat{\vector{c}}}}
\newcommand\vz{{\vector{z}}}
\newcommand\vn{{\vector{n}}}
\newcommand\vr{{\vector{r}}}
\newcommand\vsx{{\vector{s}_{\vector{x}}}}
\newcommand\vu{{\vector{u}}}
\newcommand\Cone{{C_{(1)}}}
\newcommand\Ctwo{{C_{(2)}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\RN}[1]{%
    \textup{\uppercase\expandafter{\romannumeral#1}}%
  }
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand\Nf{\mathcal{N}_\lbl{far}}
\newcommand\Ni{\mathcal{N}_\lbl{inter}}
\newcommand\Nn{\mathcal{N}_\lbl{near}}
\newcommand\Nt{\mathcal{N}_\lbl{tot}}
\newcommand\Ninit{N_\lbl{init}}

\newcommand{\Lmx}{L_{\lbl{max}}}
\newcommand{\Lmn}{L_{\lbl{min}}}
\newcommand{\ellm}{\ell_{min}}



==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler (default pdf)
##  $ make OUTOFSRC=no       #make in the same directory, otherwise inside ${BIULDDIR}
##
###

## user flags
PROJ     ?= $(notdir $(shell pwd))#defaults to dirname
OUTEXT   ?= pdf
SUMMARY  ?= grep -in --color=always "\(error\|warn\|warning\|repeated\|skipping\)"
POSTSUM  ?= awk '{ gsub("undefined", "\033[1;33m&\033[0m"); gsub("multiply defined", "\033[1;36m&\033[0m"); print }'
SYNC     ?= -synctex=1
OUTOFSRC ?= yes
BUILDDIR ?= ${_BUILDDIR}

ifeq ($(strip ${SCRATCH}),)
  _BUILDDIR = _build
else
  _BUILDDIR = ${SCRATCH}/$(strip ${PROJ})/_build
endif

ifeq ($(strip ${OUTOFSRC}),no)
  _BUILDDIR = ${CURDIR}
endif

## programs
LXX      ?= latexmk
PDFLATEX ?= pdflatex
LATEX	 ?= latex
BIBTEX	 ?= bibtex
DVI	 ?= dvipdf
PS	 ?= ps2pdf
MKDIR    ?= mkdir
OPEN     ?= open

## internal flag
LXFLAG 	 ?= -g -file-line-error -halt-on-error -shell-escape ${SYNC}
TEXFILES ?= $(shell ls -b *.tex *.bib)

ifeq (${OUTEXT},pdf)
  LXFLAG += -pdf
endif

BIBINPUTS:="..;${CURDIR};${BIBINPUTS};"
TEXINPUTS:="..;${CURDIR};${TEXINPUTS};;"

export

all: ${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})

help:
	@head -14 ${MAKEFILE_LIST}

${BUILDDIR}:
	${MKDIR} -p ${BUILDDIR}
	${MKDIR} -p ${BUILDDIR}/figs

%.${OUTEXT}:${TEXFILES} ${BUILDDIR}
	@echo "building out of source in ${BUILDDIR} for $(notdir $*)"
	cd ${BUILDDIR} && ${LXX} ${LXFLAG} ${CURDIR}/$(addsuffix .tex, $(notdir $*))
	${SUMMARY} ${BUILDDIR}/*.log ${BUILDDIR}/*.blg | ${POSTSUM}

open:
	@echo "opening ${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})"
	@${OPEN} -a /Applications/TeX/TeXShop.app ${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})

dir:
	@echo "${BUILDDIR}"

info:
	@echo "Build directory is ${BUILDDIR}"

archive:
	hg archive --include "../exclude/*" --exclude "*response.tex" $(addsuffix .tgz, ${PROJ})

clean:
	@echo "removing build directory ${BUILDDIR}"
	${RM} -r ${BUILDDIR}

.PHONY: clean open all


==> preambles.tex <==
%% use pdf 1.4 to be compatible with Elsevier requirement
\usepackage{pdf14}
\RequirePackage{snapshot} %generates a .dep file for all the dependencies

%%------------------------------------------------------------------------------
%%- Font and typesetting
%%------------------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc}
\usepackage[sc]{mathpazo}\linespread{1.05}
\usepackage[activate={true,nocompatibility},spacing,kerning]{microtype}

%%------------------------------------------------------------------------------
%%- page setup
%%------------------------------------------------------------------------------
\newlength{\alphabet}
\settowidth{\alphabet}{\normalfont abcdefghijklmnopqrstuvwxyz}
\usepackage{geometry}   %it is typically loaded by els
\geometry{textwidth=3.4\alphabet,top=1in, bottom=1.25in}
\renewcommand{\textfraction}{0.03}
\renewcommand{\topfraction}{0.95}
\renewcommand{\bottomfraction}{0.5}
%\renewcommand{\baselinestretch}{1.048}
\renewcommand{\baselinestretch}{1.0}

\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}	% require fuller float pages


%%- Math typesetting
\usepackage[fleqn,reqno]{amsmath}
\usepackage{amsfonts, amssymb, stmaryrd, xifthen}
\usepackage{mathrsfs} %% for \mathscr

%%- basic
\usepackage{xifthen}

%%- less basic
\usepackage{paralist}
%\usepackage[notref]{showkeys}

%%- referencing
\usepackage{hyperref}
\usepackage[linesnumbered,lined,ruled,vlined,commentsnumbered]{algorithm2e}
\usepackage{amsthm}
\usepackage[capitalize]{cleveref}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
% for range of refs
\crefrangelabelformat{equation}{(#3#1#4--#5#2#6)}
\crefmultiformat{equation}{Eqs.~(#2#1#3)}{ and~(#2#1#3)}{, (#2#1#3)}{, and~(#2#1#3)}
\Crefmultiformat{equation}{Equations~(#2#1#3)}{ and~(#2#1#3)}{, (#2#1#3)}{, and~(#2#1#3)}
\crefname{appendix}{}{} %els already has appendix in the name
\crefname{algocf}{Algorithm}{Algorithms} %cref refers to a counter

\crefname{heuristic}{heuristic}{heuristics}
\Crefname{heuristic}{Heuristic}{Heuristics}

%%- Floats
\usepackage{tabularx,booktabs,soul}
\usepackage[export]{adjustbox}
%\usepackage[scriptsize,tight]{subfigure}
\usepackage{subcaption}
%\usepackage[margin=10pt,font=small,textfont=it,labelfont=bf,justification=justified]{caption} %kind of collides with elsarticle class
\newcommand{\mcaption}[3]{
        \ifthenelse{\isempty{#2}}
              {\caption[#1]{\small{#3} \label{#1}}}
              {\caption[#1]{{\sc #2.} \small{#3} \label{#1}}}
        }
\newcommand{\algcaption}[3]{
        \ifthenelse{\isempty{#3}}
                   {\caption[#1]{{\sc #2.} \label{#1}}}
                   {\caption[#1]{{\sc #2.} \newline\small{#3} \label{#1}}}
        }

\usepackage{graphicx}
\graphicspath{{figs/}}
\newcommand\cbox[2][.4\linewidth]{\parbox[t]{#1}{#2}}
\usepackage{multirow}
\usepackage[margin=10pt,font=small,textfont=it,labelfont=bf,justification=justified]{caption}

\usepackage{titlesec}
\titleformat{\subsubsection}[runin]{\normalfont\normalsize\itshape}{\thesubsubsection.}{.5em}{}[.\hspace{.5em}]
\titleformat{\paragraph}[runin]{\normalfont\normalsize\itshape}{\theparagraph}{}{}[.\hspace{.5em}]

%%- Miscelenous packages
\usepackage[normal]{engord} %remove normal option to have raised suffix
\usepackage{bm, ifdraft, paralist}

\usepackage{tikz,pgf}
\usepackage{pgfplots}
\usepackage{ctable}
\newcommand{\includepgf}[2][1]{
      \beginpgfgraphicnamed{#2}%
        \scalebox{#1}{}%
      \endpgfgraphicnamed%
}

%%- typography
\newcommand\para[1]{\paragraph*{#1}}
\newcommand\lh[1]{\emph{#1}}%line heading
\newcommand\mbf[1]{\ensuremath{\mathbf{#1}}}
\newcommand\attn[1]{\hl{\textbf{#1}}}
\newcommand\comment[1]{\ifdraft{\textcolor{orange}{[\textbf{Draft comment:} #1]}}{}}
\newcommand\note[2][DRAFT]{\ifoptionfinal{}{\textcolor{magenta}{[\textbf{#1:} #2]}}}
\newcommand\lbl[1]{\ensuremath{\mathrm{#1}}}

%%- new math operators
\def\D{\ensuremath{\,d}}
\def\defeq{\mathrel{\mathop :}=}
\def\eps{\epsilon}
\newcommand\norm[2][{}]{\lVert #2 \rVert_{#1}}
\newcommand\jump[1]{\llbracket #1 \rrbracket}
\newcommand\ord[1]{\ensuremath{\mathcal{O}\left(#1\right)}}

\newcommand\ordinal[1]{\ifthenelse{\isin{#1}{abcdefghijklmnopqrstuvwxyz}}{\ensuremath{#1^\mathrm{th}}}{\engordnumber{#1}}}
\newcommand\scalar[1]{\ensuremath{#1}}
\renewcommand\vec[1]{\ensuremath{#1}}
\newcommand\op[1]{\ensuremath{\mathcal #1}}
\newcommand\disc[2]{\ensuremath{\bm{\mathsf{#1}}}}
\newcommand\parderiv[2]{\frac{\partial #1}{\partial #2}}

%%- proofreading
\usepackage{soul,marginnote,todonotes,cprotect}
%\leavevmode\color{blue}[#1]}
%\newcommand\edit[2]{\textcolor{gray}{#1}\ \textcolor{magenta}{#2}}
\newcommand\edit[2]{\textcolor{gray}{#1}\ \leavevmode\color{magenta}#2\color{black}}
\newcommand\editone[2]{\textcolor{gray}{#1}\ \textcolor{orange}{#2}}
\newcommand\editt[2]{\edit{\st{#1}}{#2}}
\newcommand\editm[2]{\textcolor{gray}{\ensuremath{#1}}\ \textcolor{magenta}{\ensuremath{#2}}}
\newcommand\edittxt[2]{\editt{#1}{#2}}
\newcommand\editmath[2]{\editm{#1}{#2}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{heuristic}[theorem]{Heuristic}

\usepackage{enumitem}
\newlist{criteria}{enumerate}{10}
\setlist[criteria]{label*=\arabic*}


\crefname{criteriai}{Criterion}{Criteria}
\Crefname{criteriai}{Criterion}{Criteria}
\crefname{alg}{algorithm}{algorithms}
\Crefname{alg}{Algorithm}{Algorithms}
\newcommand{\DZ}[1]{\textcolor{blue}{#1}}
\newcommand{\Res}[1]{\textcolor{blue}{#1}}

\input{macros}

\newlength\figureheight
\newlength\figurewidth




